On User-Level Private Convex Optimization

We introduce a new mechanism for stochastic convex optimization (SCO) with user-level differential privacy guarantees. The convergence rates of this mechanism are similar to those in the prior work of Levy et al. (2021); Narayanan et al. (2022), but with two important improvements. Our mechanism does not require any smoothness assumptions on the loss. Furthermore, our bounds are also the first where the minimum number of users needed for user-level privacy has no dependence on the dimension and only a logarithmic dependence on the desired excess error. The main idea underlying the new mechanism is to show that the optimizers of strongly convex losses have low local deletion sensitivity, along with an output perturbation method for functions with low local deletion sensitivity, which could be of independent interest.

==> app-sgd-unused.tex <==
\section{(S)GD-Based Algorithms}

\pasin{This section is mostly for my own sanity...}

\subsection{Additional Preliminaries}

Recall that a scalar random variable $X$ is said to be \emph{$\sigma^2$-sub-Gaussian} iff $\E[\exp(X - \E[X])] \leq \exp(\sigma^2 / 2)$. Furthermore, we say that a vector random variable $\bv$ is \emph{$\sigma^2$-sub-Gaussian} iff $\left<\bv, \bu\right>$ is $\sigma^2$-sub-Gaussian for all $\bu \in \cB_d(1)$.

We say that two distributions (or corresponding random variables) $\cD_0, \cD_1$ are $\beta$-close if their total variation distance is at most $\beta$.

We say that a vector-valued random variable $\hbu$ is an \emph{unbiased estimator of $\bu \in \R^d$ with variance $\sigma^2$} iff $\E[\hbu] = \bu$ and $\E[\|\hbu - \bu\|_2^2] \leq \sigma^2$.

\subsection{Adaptive Linear Queries with User-Level DP}

Let $n, m, k \in \N$ be any positive integers.

We consider the following adaptive linear queries problem. Let $\{f_\theta\}_{\theta \in \Theta}$ be a family of queries, where $f_{\theta}: \cX \to \R^d$. Suppose that there are $n$ users, and let the input to the $i$-th user be $x_{i, 1}, \dots, x_{i, m}$ drawn i.i.d. from $\cD$. Let $f_{\theta}(\bx)$ be defined as $\frac{1}{nm} \sum_{i \in [n]} \sum_{j \in [m]} f_\theta(x_{i, j})$ Furthermore, assume that for every $\theta \in \Theta$,  $\|f_{\theta}(x)\| \leq G$. Our goal is to output estimates for\footnote{Note that this is the \emph{empricial} value of linear query. A similar result holds for distribution version by applying a concentration inequality.} $f_{\theta_1}(\bx), \dots, f_{\theta_k}(\bx)$, where $\theta_1, \dots, \theta_k$ are chosen adaptively (i.e. $\theta_i$ can depend on the answers to the previous queries).

\begin{theorem} \label{thm:adaptive-lin-queries}
Assuming that $n \geq \tO(1/\eps)$ and that $\|f_{\theta}(x)\| \leq G$. Then, there exists an $(\eps, \delta)$-DP algorithm for answering $k$ adaptive linear queries such that for each query $\theta_i$, it produces an estimator that is $\beta$-close to an unbiased estimator with variance $\sigma_{lin}^2$ where $\sigma_{lin} \leq \tO\inparen{\frac{G \sqrt{k}}{\eps n\sqrt{m}}}.$
\end{theorem}

\begin{proof}[Proof Sketch]
We use $\bx^i$ to denote the dataset of the $i$-th user, i.e. $\bx^{i} := (x_{i, 1}, \dots, x_{i, m})$.
Let $\eps' = \tOmega(\eps/\sqrt{k}), \delta' = \tOmega(\delta/k)$ be such that $k$-fold advanced composition of $(\eps', \delta')$-DP algorithms is $(\eps, \delta)$-DP.

The algorithm is simple: when answering the $i$-th query, just use $(\eps', \delta')$-DP for \Cref{thm:mean-est} with $\tau = \tO(G/\sqrt{m})$. We note that the variance bound from \Cref{thm:mean-est} immediately implies the claimed bound, \emph{assuming that $f_{\theta_\ell}(\bx^1), \dots, f_{\theta_\ell}(\bx^n)$ lie within a ball of radius $\tau$ for all $\ell \in [n]$ w.h.p.}

Finally, we will now prove why the italic statement in above holds. First, by union boud, we have
\begin{align*}
&\Pr[\forall \ell \in [k], f_{\theta_\ell}(\bx^1), \dots, f_{\theta_\ell}(\bx^n) \text{ lie within a ball of radius } \tau] \\
&\leq \sum_{\ell \in [k]} \sum_{i \in [n]} \Pr[\|f_{\theta_\ell}(\bx^i) - f_{\theta_\ell}(\cD) \| \leq \tau/2].
\end{align*}
Now, the only issue with bounding $\Pr[\|f_{\theta_\ell}(\bx^i) - f_{\theta_\ell}(\cD) \| \leq \tau/2]$ is that $\theta_\ell$ is dependent on $\bx^i$ (through previous linear query answers given by the algorithm). To be more precise, let $\cP_\ell(\bx^1, \dots, \bx^n)$ denote the distribution of $\theta_\ell$ when inputs are $\bx^1, \dots, \bx^n$. Let $\bx'^i$ denote an arbitrary $m$-size dataset. Using the fact that the algorithm is $(\eps,\delta)$-DP, we have
\begin{align*}
&\Pr[\|f_{\theta_\ell}(\bx^i) - f_{\theta_\ell}(\cD) \| \leq \tau/2] \\
&= \Pr_{(\bx^i) \sim \cD^{\otimes m}}\Pr_{\theta_\ell \sim \cP_\ell(\bx^1, \dots, \bx^n)}[\|f_{\theta_\ell}(\bx^i) - f_{\theta_\ell}(\cD) \| \leq \tau/2] \\
&\leq e^{\eps} \Pr_{(\bx^i) \sim \cD^{\otimes m}}\Pr_{\theta_\ell \sim \cP_\ell(\bx^1, \dots, \bx^{j-1}, \bx'^{j}, \bx^{j + 1}, \bx^n)}[\|f_{\theta_\ell}(\bx^i) - f_{\theta_\ell}(\cD) \| \leq \tau/2] + \delta \\
&=  e^{\eps} \Pr_{\theta_\ell \sim \cP_\ell(\bx^1, \dots, \bx^{j-1}, \bx'^{j}, \bx^{j + 1}, \bx^n)}\Pr_{(\bx^i) \sim \cD^{\otimes m}}[\|f_{\theta_\ell}(\bx^i) - f_{\theta_\ell}(\cD) \| \leq \tau/2] + \delta,
\end{align*}
where the last exchange follows from the fact that $\cP_\ell(\bx^1, \dots, \bx^{j-1}, \bx'^{j}, \bx^{j + 1}, \bx^n)$ does not depend on $\bx^j$.
We can then finish the proof by observing that for any fixed $\theta$, $\Pr_{(\bx^i) \sim \cD^{\otimes m}}[\|f_{\theta}(\bx^i) - f_{\theta_\ell}(\cD) \| \leq \tau/2]$ is $(nk)^{-\omega(1)}$ due to standard concentration bound.
\end{proof}

\subsection{Gradient Descent-Based Algorithms with User-Level DP}

Below we state a generic form of the theorem based on gradient descent alone; this should be compared with \cite[Theorem 4]{LevySAKKMS21} and the subsequent improvement \cite[]{NarayananME22}. The $T$-independent terms we get below are as good as their bounds \emph{but we do not require smoothness}. However, the first term (i.e. convergence rate) is larger (i.e. slower); this seems inevitable since without smoothness the bounds we get are already the best bounds possible in terms of $T$ for first order optimization even without privacy.

\pasin{The strongly convex bound is not used anywhere later in the write-up, so please feel free to ignore them for now.}




\subsubsection{Generic Noisy (S)GD Guarantees}

The following theorem is well-known.
\pasin{TODO: Find the right citations...}

\begin{theorem}[{\cite[Theorem 6.1]{Bubeck15}}] \label{thm:first-order-opt-generic}
Let $\bx$ be any dataset. Suppose that there exists an oracle (which will be called in $T$ adaptive queries) that, on input $\theta$, can output $\tg(\theta)$ such that $\E[\tg(\theta)] \in \nabla \cL(\theta; \bx)$ and $\E[\|\tg(\theta)\|^2] \leq B^2$.
\begin{itemize}
\item If $\ell$ is convex, then there exists an algorithm that outputs $\htheta$ such that
\begin{align*}
\E[\cL(\htheta; \cX)] - \min_{\theta'} \cL(\theta'; \cX) \leq O(R B/\sqrt{T}).
\end{align*}
\item If $\ell$ is $\mu$-strongly convex, then there exists an algorithm that outputs $\htheta$ such that
\begin{align*}
\E[\cL(\htheta; \cX)] - \min_{\theta'} \cL(\theta'; \cX) \leq O\inparen{\frac{B^2}{\mu T}}.
\end{align*}
\end{itemize}
\end{theorem}

\subsubsection{Mean Estimation}

In the mean estimation problem, there are $N$ vectors $\bv_1, \dots, \bv_{N}$. The goal is to output an estimate of $\frac{1}{N} \sum_{i \in [N]} \bv_i$.

The following can be derived from~\cite{NarayananME22,TsfadiaCKMS22}.

\begin{theorem} \label{thm:mean-est}
Suppose $N \geq \tO(1/\eps)$.
For any $\beta > 0$, there exists an $(\eps,\delta)$-DP algorithm that, when $\bv_1, \dots, \bv_N$ all lie within a ball of radius $\tau$, it outputs an estimator that is $\beta$-close to an unbiased estimator with variance $\tilde{O}\inparen{\frac{d \cdot \tau^2}{\eps^2 N^2}}$.
\end{theorem}

\pasin{Note that the above papers actually do not claim unbiasedness. In fact,~\cite{NarayananME22} is pretty clearly biased. So this might require some modification, but it should be true.}

\begin{theorem} 
For any $T \in \N, \eps, \delta \in (0, 1)$, suppose that $n > \tO(\sqrt{T}/\eps)$. Suppose that $\ell$ is $G$-Lipschitz.
\begin{itemize}
\item If $\ell$ is convex, then there exists an $(\eps, \delta)$-DP algorithm that outputs $\htheta$ such that
\begin{align*}
\E[\cL(\htheta; \bx)] - \min_{\theta'} \cL(\theta'; \bx) \leq \tO\inparen{\frac{GR}{\sqrt{T}} + \frac{G R \sqrt{d}}{\eps n \sqrt{m}}}.
\end{align*}
\item If $\ell$ is $\mu$-strongly convex, then there exists an $(\eps, \delta)$-DP algorithm that outputs $\htheta$ such that
\begin{align*}
\E[\cL(\htheta; \bx)] - \min_{\theta'} \cL(\theta'; \bx) \leq \tO\inparen{\frac{G^2}{\mu T} + \frac{G d}{\eps n^2 m}}.
\end{align*}
\end{itemize}
\end{theorem}

\begin{proof}[Proof Sketch]
This is a simple combination between \Cref{thm:first-order-opt-generic} and \Cref{thm:adaptive-lin-queries}. Specifically, applying the latter (with $k = T$) gives $B \leq \tO\inparen{G + \frac{d\sigma\sqrt{k}}{\eps n\sqrt{m}}} = \tO\inparen{G + \frac{G\sqrt{d T}}{\eps n\sqrt{m}}}$ where the $G$ term is due to the norm of the (non-noisy) gradient itself. Plugging this into \Cref{thm:first-order-opt-generic} then yields the claimed bounds.
\end{proof}

\pasin{Note that the problem with the above theorem is that in the as that we (roughly) fix $n$ and let $m \to \infty$, we can still run GD only for a function of $n$ steps. This means that the excess risk bound will not go to zero.}
